Ranked Enumeration of Join Queries with Projections

Join query evaluation with ordering is a fundamental data processing task in relational database management systems. SQL and custom graph query languages such as Cypher offer this functionality by allowing users to specify the order via the ORDER BY clause. In many scenarios, the users also want to see the first $k$ results quickly (expressed by the LIMIT clause), but the value of $k$ is not predetermined as user queries are arriving in an online fashion. Recent work has made considerable progress in identifying optimal algorithms for ranked enumeration of join queries that do not contain any projections. In this paper, we initiate the study of the problem of enumerating results in ranked order for queries with projections. Our main result shows that for any acyclic query, it is possible to obtain a near-linear (in the size of the database) delay algorithm after only a linear time preprocessing step for two important ranking functions: sum and lexicographic ordering. For a practical subset of acyclic queries known as star queries, we show an even stronger result that allows a user to obtain a smooth tradeoff between faster answering time guarantees using more preprocessing time. Our results are also extensible to queries containing cycles and unions. We also perform a comprehensive experimental evaluation to demonstrate that our algorithms, which are simple to implement, improve up to three orders of magnitude in the running time over state-of-the-art algorithms implemented within open-source RDBMS and specialized graph databases.

==> experiments.tex <==
\section{Experimental Evaluation} \label{sec:experiments}

In this section, we perform an extensive evaluation of our proposed algorithm. Our goal is to evaluate three aspects: $(a)$ how fast our algorithm is compared to state-of-the-art implementations for both \SUM\ and \lexi\ ranking functions on various queries, $(b)$ test the empirical performance of the space-time tradeoff in~\autoref{thm:ranked:star} and $(c)$ investigate the performance of our algorithm on UCQs, cycles and whether the theoretically claimed guarantee of linear delay actually holds in practice.

\subsection{Experimental Setup}

We use Neo4j $4.2.3$ community edition, MariaDB $10.1.47$\footnote{Compared with MySQL, MariaDB performed better in our experiments, hence we report the results for MariaDB} and PostgreSQL $11.12$ for our experiments. All experiments are performed on a Cloudlab machine~\cite{duplyakin2019design} running Ubuntu $18.04$ equipped with two Intel E5-2630 v3 8-core CPUs@$2.40$ GHz and $128$ GB RAM. We focus only on the main memory setting and all experiments run on a single core. Since the join queries are memory intensive, we take special care to ensure that only one DBMS engine is running at a time, restart the session for each query to ensure temp tables in main memory are flushed out to avoid any interference, and also monitor that no temp tables are created on the disk. We only keep one database containing a single relation when performing experiments. We switch off all logging to avoid any performance impact. For PostgreSQL and MariaDB, we allow the engines to use the full main memory to ensure all temp tables are resident in the RAM and sorting (if any) happens without any disk IOs by increasing the sort buffer limit. For Neo4j, we allow the JVM heap to use the full main memory at the time of start up. We also build bidirectional B-tree indexes for each relation ahead of time and create named indexes in Neo4j. All of our algorithms are implemented in C++ and compiled using the GNU C++ $7.5.0$ compiler that ships with Ubuntu $18.04$. Each experiment is run $5$ times and we report the median after removing the slowest and the fastest run.

\begin{figure*}[!htp]
	\begin{subfigure}{0.24\linewidth}
		\hspace*{-1em}
		\includegraphics[scale=0.17]{figures/dblpsumvaryingknopreprocessing.pdf}
		\caption{DBLP $\twopath$}  \label{fig:dblp:2path}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\vspace*{-1.2em}
		\hspace*{-1.25em}
		\includegraphics[scale=0.17]{figures/dblp3pathsumvaryingknopreprocessing.pdf}
		\caption{DBLP $\threepath$}  \label{fig:dblp:3path}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/dblp4pathsumvaryingknopreprocessing.pdf}
		\caption{DBLP $\fourpath$}  \label{fig:dblp:4path}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/dblp3starsumvaryingknopreprocessing.pdf}
		\caption{DBLP $\threestar$}  \label{fig:dblp:3star}
	\end{subfigure}
	
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/imdbsumvaryingknopreprocessing.pdf}
		\caption{IMDB $\twopath$}  \label{fig:imdb:2path}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/imdb3pathsumvaryingknopreprocessing.pdf}
		\caption{IMDB $\threepath$}  \label{fig:imdb:3path}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/imdb4pathsumvaryingknopreprocessing.pdf}
		\caption{IMDB $\fourpath$}  \label{fig:imdb:4path}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/imdb3starsumvaryingknopreprocessing.pdf}
		\caption{IMDB $\threestar$}  \label{fig:imdb:3star}
	\end{subfigure}
	\caption{Comparing our linear delay algorithm with state-of-the-art engines for sum function} \label{fig:linear:notradeoff}
\end{figure*}

\begin{figure*}[!htp]
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/dblplexicographicvaryingknopreprocessing.pdf}
		\caption{DBLP $\twopath$}  \label{fig:dblp:2path:lex}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/dblp3pathlexicographicvaryingknopreprocessing.pdf}
		\caption{DBLP $\threepath$}  \label{fig:dblp:3path:lex}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/dblp4pathlexicographicvaryingknopreprocessing.pdf}
		\caption{DBLP $\fourpath$}  \label{fig:dblp:4path:lex}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/dblp3starlexicographicvaryingknopreprocessing.pdf}
		\caption{DBLP $\threestar$}  \label{fig:dblp:3star:lex}
	\end{subfigure}
	
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/imdblexicographicvaryingknopreprocessing.pdf}
		\caption{IMDB $\twopath$}  \label{fig:imdb:2path:lex}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/imdb3pathlexicographicvaryingknopreprocessing.pdf}
		\caption{IMDB $\threepath$}  \label{fig:imdb:3path:lex}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/imdb4pathlexicographicvaryingknopreprocessing.pdf}
		\caption{IMDB $\fourpath$}  \label{fig:imdb:4path:lex}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/imdb3starlexicographicvaryingknopreprocessing.pdf}
		\caption{IMDB $\threestar$}  \label{fig:imdb:3star:lex}
	\end{subfigure}
	\caption{Comparing our linear delay algorithm with state-of-the-art engines for lexicographic function.} \label{fig:linear:notradeoff:lex}
\end{figure*}

\smallskip
\introparagraph{Datasets} We use two real world datasets for our experiments: the DBLP dataset, a binary relation containing relationship between authors and papers, and the IMDB dataset, a binary relation containing actors and movies.~\autoref{table:workload:characteristics} shows the important parameters of the dataset. For each vertex, we assign a unique value as an ID that acts as the weight over which the ranking function is defined.


\begin{table} \centering
	%\ra{1.3}
	\begin{small}
		\begin{tabular}{@{}rrrcr@{}}\toprule
			\textbf{dataset} & \textbf{\#edges} & \textbf{\#nodes} & \textbf{max/avg degree}  & \textbf{weights} \\ \midrule
			DBLP & 1,049,866 & 189114 & 306/5.55 & random  \\ 
			IMDB & 7,523,205 & 2746447 & 1623/2.73 & random    \\ 
			\bottomrule
		\end{tabular}
	\end{small}
	\caption{Dataset characteristics}
	\label{table:workload:characteristics}
\end{table}

\smallskip
\introparagraph{Queries} We consider $4$ join queries as shown below for the binary relation $R(A,B)$, which are  commonly seen in practice~\cite{bonifati2020analytical}. Function $w(A)$ is the weight function defining on vertex.

\begin{lstlisting}[language=SQL,
deletekeywords={IDENTITY},
deletekeywords={[2]INT},
morekeywords={clustered},
mathescape=true,
xleftmargin=0pt,
framexleftmargin=0pt,
frame=tb,
framerule=0pt ]

$\twopath$ = SELECT DISTINCT $R_1.A, R_2.A$ FROM $R$ AS $R_1$, $R$ AS $R_2$
WHERE $R_1.B = R_2.B$ ORDER BY f(w($R_1.A$), w($R_2.A$)) LIMIT k;

$\threepath$ = SELECT DISTINCT $R_1.A, R_3.B$ FROM $R$ AS $R_1$, $R$ AS $R_2$, 
$R$ AS $R_3$ WHERE $R_1.B = R_2.B$ AND $R_2.A = R_3.A$ ORDER BY 
f(w($R_1.A$), w($R_3.B$)) LIMIT k;

$\fourpath$ = SELECT DISTINCT $R_1.A, R_4.A$ FROM $R$ AS $R_1$, $R$ AS $R_2$, 
$R$ AS $R_3$, $R$ AS $R_4$ WHERE $R_1.B = R_2.B$ AND $R_2.A = R_3.A$  AND 
$R_3.B = R_4.B$ ORDER BY f(w($R_1.A$),w($R_4.A$)) LIMIT k;

$\threestar$ = SELECT DISTINCT $R_1.A, R_2.A, R_3.A$ FROM $R$ AS $R_1$, $R$ AS 
$R_2$, $R$ AS $R_3$ WHERE $R_1.B = R_2.B$ AND $R_2.B = R_3.B$ ORDER BY 
f(w($R_1.A$),w($R_2.A$),w($R_3.A$)) LIMIT k;
\end{lstlisting}


\subsection{Linear Delay Algorithm} \label{thm1:exp}

In this section, we compare the empirical performance of the algorithm given by~\autoref{thm:general} (labeled as \textsc{LinDelay} in all figures) against the baselines for each query. In order to perform a fair comparison, we materialize the top-$k$ answers in-memory since other engines also do it. However, a strength of our system is that if a downstream task only requires the output as a stream, we are able to enumerate the result instead of materializing it, which is not possible with other engines. Further, for all queries executed on DBMS engines and Neo4j, we explicitly set \sqlhighlight{LIMIT 10} to retrieve the top-$10$ answers in all our experiments. This is done to ensure that there is no overhead of outputting answers to console or a file and avoid pagination of the output, which are expensive operations and impacts the total running time. Further, this also lets us measure the delay between submitting the query and getting the first few answers. Obviously, for a value of \sqlhighlight{LIMIT} larger than $10$, the engines will require even more time, so the performance numbers reported here are lower bounds to the actual running time for larger $k$.

\smallskip
\introparagraph{Sum ordering} \autoref{fig:linear:notradeoff} shows the main results for the DBLP and IMDB datasets when the ranking function is the sum function. Let us first review the results for the DBLP dataset. \autoref{fig:dblp:2path} shows the running time for different values of $k$ in the limit clause. The first observation is that all engines materialize the join result, followed by deduplicating and sorting according to the ranking function which leads to poor performance for all baselines. This is because all engines treat sorting and distinct clause as blocking operators, verified by examining the query plan. On the other hand, our approach is limit-aware. For small values of $k$, we are up to two orders of magnitude faster and as the value of $k$ increases, the total running time of our algorithm increases linearly. Even when our algorithm has to enumerate and materialize the entire result, it is still faster than asking the engines for the top-$10$ results. This is a direct benefit of generating the output in deduplicated and ranked order. As the path length increases from two to three and four path (\autoref{fig:dblp:3path} and \autoref{fig:dblp:4path}), the performance gap between existing engines and our approach also becomes larger.  We also point out that all engines require a large amount of main memory for query execution. For example, MariaDB requires about $40$GB of memory for executing $\fourpath$ on DBLP. In contrast, the space overhead of our algorithm is dominated by the size of the priority queue. For DBLP dataset, our approach requires a measly $1.3$GB, $4$GB, $3$GB and $2.7$GB total space for $\twopath, \threepath, \fourpath$ and $\threestar$ respectively. For $\threepath, \fourpath$ and $\threestar$, we also implement breadth first search (BFS) followed by a sorting step using the idea of~\autoref{algo:lexicographic}. As it can be seen from the figures, BFS and sort provides an intermediate strategy which is faster than our algorithm for large values of $k$ but at the cost of expensive materialization of the entire result, which may not be always possible (and is the case for IMDB dataset). However, deciding to use BFS and sort requires knowledge of the output result size, which is unknown apriori and difficult to estimate.



For the IMDB dataset, we observe a similar trend of our algorithm displaying superior performance compared to all other baselines. In this case, BFS and sorting even for $\fourpath$ is not possible since the result is almost $0.5$ trillion items. For $\threestar$, none of the engines were able to compute the result after running for $5$ hours when main memory ran out. BFS and sort also failed due to the size being larger than the main memory limit. Lastly, Neo4j was consistently the best performing (albeit marginally) engine among all baselines. While there is little scope for rewriting the SQL queries to try to obtain better performance, Neo4j has graph-specific operators such as variable length expansion. We tested multiple rewritings of the query, which leads to different query plans, to obtain the best performance (although this is the job of the query optimizer), which is finally reported in the figures. Regardless of the rewritings, Neo4j still treats materializing and sorting as a blocking operator which is a fundamental bottleneck.

\begin{figure*}[!tp]
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/dblpsumvfixedkvaryingpreprocessingandspace.pdf}
		\caption{DBLP $\twopath$}  \label{fig:dblp:2path:tradeoff}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\vspace*{-1.4em}
		\includegraphics[scale=0.17]{figures/imdbsumvfixedkvaryingpreprocessingandspace.pdf}
		\caption{IMDB $\twopath$}  \label{fig:imdb:2path:tradeoff}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/dblp3starsumvfixedkvaryingpreprocessingandspace.pdf}
		\caption{DBLP $\threestar$}  \label{fig:dblp:3star:tradeoff}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/imdb3starsumvfixedkvaryingpreprocessingandspace.pdf}
		\caption{IMDB $\threestar$}  \label{fig:imdb:3star:tradeoff}
	\end{subfigure}
	\caption{Comparing the preprocessing and enumeration tradeoff for sum function when enumerating the entire result} \label{fig:linear:tradeoff}
\end{figure*}

\begin{figure*}[!htp]
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/dblplexicographicfixedkvaryingpreprocessingandspace.pdf}
		\caption{DBLP $\twopath$}  \label{fig:dblp:2path:tradeoff:lex}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/dblp3starlexicographicvfixedkvaryingpreprocessingandspace.pdf}
		\caption{DBLP $\threestar$}  \label{fig:dblp:3star:tradeoff:lex}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/imdblexicographicfixedkvaryingpreprocessingandspace.pdf}
		\caption{IMDB $\twopath$}  \label{fig:imdb:2path:tradeoff:lex}
	\end{subfigure}
	\begin{subfigure}{0.24\linewidth}
		\includegraphics[scale=0.17]{figures/imdb3starlexicographicvfixedkvaryingpreprocessingandspace.pdf}
		\caption{IMDB $\threestar$}  \label{fig:imdb:3star:tradeoff:lex}
	\end{subfigure}
	\caption{Comparing the preprocessing and enumeration tradeoff for lexicographic function when enumerating the entire result} \label{fig:linear:tradeoff:lex}
\end{figure*}

\smallskip
\introparagraph{Lexicographic ordering} \autoref{fig:dblp:2path:lex},\ref{fig:dblp:3path:lex},\ref{fig:dblp:4path:lex} and \ref{fig:dblp:3star:lex} show the running time for different values of $k$ in the limit clause for lexicographic ranking function on DBLP. The first striking observation here is that the running time for all baseline engines is identical to that of sum function. This demonstrates that existing engines are also agnostic to the ranking function in the query and fail to take advantage of the additional structure. However, lexicographic functions are easier to handle in practice than sum because we can avoid the use of a priority queue altogether. This in turn leads to faster running time since push and pops from the priority queue are expensive due to the logarithmic overhead and need for re-balancing of the tree structure. Thus, we obtain a $2\times$ improvement for lexicographic ordering as compared to the sum function.  \autoref{fig:imdb:2path:lex},\ref{fig:imdb:3path:lex},\ref{fig:imdb:4path:lex} and \ref{fig:imdb:3star:lex} show the results for the IMDB dataset. For $\threepath$ and $\fourpath$, no other engine was able to perform the join computation within the cutoff time of $5$ hours.

\smallskip
\introparagraph{Measuring the delay} Our final experiment in this subsection evaluates how many priority queue operations are required for each answer tuple. Recall that for each answer, our algorithm performs $O(|D|)$ priority queue operations in the worst-case (\autoref{thm:general}). Thus, the number of priority queue operations is a proxy for the delay between any two answers. \autoref{delay} plots the fraction of answers that require a certain number of PQ operations for $\twopath$ on DBLP. Nearly $70\%$ of answers require only one PQ push and pop operation and $99\%$ of the output requires at most $22$ push and pop operations. However, there are some outliers as well. The largest number of push and pops over all answers is $306$. This is not particularly surprising given the fact that DBLP is a sparse dataset but dense matrix datasets can easily have a large duplication in practice. For the IMDB dataset, we found that $95\%$ of answers require one priority queue operation and $99\%$ of answers needed at most three operations.


\subsection{Enumeration with Preprocessing} \label{sec:preprocess}

In this section, we investigate the empirical performance of the preprocessing step and its impact on the result enumeration as described by~\autoref{thm:ranked:star}. For all experiments in this section, we fix $k$ to be large enough to enumerate the entire result (which is equivalent to having no limit clause at all).


\smallskip
\introparagraph{Sum ordering} \autoref{fig:dblp:2path:tradeoff} and \autoref{fig:imdb:2path:tradeoff} show the tradeoff between space used by the data structure constructed in the preprocessing phase and running time of the enumeration algorithm for $\twopath$ on DBLP and IMDB repectively. We show the tradeoff for $6$ different space budgets but the user is free to choose any space budget in the entire spectrum. As expected, the time required to enumerate the result is large when there is no preprocessing and it gradually drops as more and more results are materialized in the preprocessing phase. The sum of preprocessing time and enumeration time is not a flat line: this is because as an optimization, we do not use priority queues in the preprocessing phase. Instead, we can simply use the BFS and sort algorithm for all chosen nodes which need to be materialized. This is a faster approach in practice as we avoid use of priority queues but priority queues cannot be avoided for enumeration phase. We observe similar trend for $\threestar$ on both datasets as well. 

\begin{figure*}
	\begin{subfigure}{0.33\linewidth}
		\includegraphics[scale=0.2]{figures/cdfpop.pdf}
		\caption{DBLP $\twopath$ \pq\ operations per answer}  \label{delay}
	\end{subfigure}
	\begin{subfigure}{0.33\linewidth}
		\includegraphics[scale=0.2]{figures/dblpsumfourcycle.pdf}
		\caption{DBLP 4-cycle enumeration for sum} \label{enum:4cycle}
	\end{subfigure}
	\begin{subfigure}{0.33\linewidth}
		\includegraphics[scale=0.2]{figures/ucq24pathsumvaryingknopreprocessing.pdf}
		\caption{DBLP $\twopath \cup \fourpath$ for sum} \label{ucq}
	\end{subfigure}
	\caption{Measuring the delay guarantee in practice and performance for 4-cycle and UCQs for DBLP dataset}
\end{figure*}

\begin{figure}
	\includegraphics[scale=0.2]{figures/imdbsumvaryingkfixedpreprocessingwithtotalenum.pdf}
	\caption{IMDB enumeration with and without preprocessing for sum function} \label{enum:tradeoff}
\end{figure}

At this point, the reader may wonder about the following question: under what circumstances should preprocessing be done? There are two aspects to this decision. First, if the value of $k$ in the limit clause is known and it is small, there may not be a need to perform preprocessing. Let us examine this using~\autoref{enum:tradeoff} that shows the enumeration time with and without preprocessing when we fix the materialization space budget to $8$GB. If $k = 10^6$, then enumerating the results without any preprocessing takes $2$ seconds. But creating the data structure takes $27$ seconds. In this scenario, performing an expensive preprocessing step is not beneficial directly. However, if a downstream task requires repeated enumeration of the query result, performing a preprocessing phase is beneficial since the enumeration time becomes smaller as we materialize more output ahead of time. If multiple consumers ask for the $\twopath$ result repeatedly, a preprocessing phase can reduce the enumeration time drastically. We illustrate this with a concrete example. Suppose that a downstream task needs to enumerate the entire result (which means $k = 1.8 \cdot 10^8$) $10$ times. Let us fix the space budget for materialization as $8$GB. Constructing this data structure requires $27$ seconds as a one-time cost and enumeration using this data structure takes $42$ seconds. Thus, enumerating the result $10$ times requires $42 \cdot 10 +27 = 447$ seconds in total. On the other hand, the \textsc{LinDelay} algorithm enumerates the result in $102$ seconds without any data structure. Thus, enumerating $10$ times requires $102 \cdot 10$ seconds, which is slower as compared to when we use the data structure. As $k$ becomes smaller, the threshold for number of times a query result must be repeatedly enumerated becomes larger, which impacts the decision to whether preprocessing is required or not.

\smallskip
\introparagraph{Lexicographic ordering} \autoref{fig:dblp:2path:tradeoff:lex}, \ref{fig:dblp:3star:tradeoff:lex} show the results for $\twopath$ and $\threestar$ on DBLP for lexicographic ordering. Compared to the sum function, there is a smooth tradeoff between preprocessing time and enumeration time. This is because the algorithm used for preprocessing and enumeration is identical (both of them do not use any priority queues), which leads to a flatter total time (green line with circle marker). Once again, as more results are materialized in the preprocessing phase, enumeration becomes faster. The same conclusions hold for the IMDB dataset (\autoref{fig:imdb:2path:tradeoff:lex}, \ref{fig:imdb:3star:tradeoff:lex}).


%\begin{figure}
%	\includegraphics[scale=0.22]{figures/imdbsumvaryingkfixedpreprocessingwithtotalenum.pdf}
%	\caption{IMDB enumeration with and without preprocesing for sum function} \label{enum:tradeoff}
%\end{figure}
%\begin{figure}
%	\includegraphics[scale=0.22]{figures/ucq24pathsumvaryingknopreprocessing.pdf}
%	\caption{DBLP $\twopath \cup \fourpath$ for sum function} \label{ucq}
%\end{figure}

\subsection{Extension to UCQs and Cyclic Queries}

In this section, we evaluate the empirical performance of the UCQ $\twopath \cup \fourpath$ for different values of $k$ in the \sqlhighlight{LIMIT} clause for \textsc{LinDelay}. For all baselines, we explicitly set \sqlhighlight{LIMIT 10}. The ranking function as sum. Due to lack of space, we only present the results for the DBLP dataset (\autoref{ucq}). Similar to the other experiments, all engines provide poor performance since they evaluate each fragment of the UCQ in isolation followed by a final merge step and then sorting. Our algorithm combines the sorted output from all UCQs in a non-blocking fashion. This approach of on-the-fly merging also reduces the space requirement of the algorithm since we are materializing only the deduplicated output. In contrast, if any of the subqueries in a UCQ require large space for materialization, none of the engines will be able to execute the query in a reasonable amount of time. Finally, in order to test the empirical performance for cyclic queries, we choose the following 4-cycle query on DBLP.

\begin{lstlisting}[language=SQL,
deletekeywords={IDENTITY},
deletekeywords={[2]INT},
morekeywords={clustered},
mathescape=true,
xleftmargin=0pt,
framexleftmargin=0pt,
frame=tb,
framerule=0pt ]
$Q_\textsf{4cycle}$ = SELECT DISTINCT $R_1.A, R_4.A$ FROM $R$ AS $R_1$, $R$ AS $R_2$, 
$R$ AS $R_3$, $R$ AS $R_4$ WHERE $R_1.B = R_2.B$ AND $R_2.A = R_4.A$ AND 
$R_3.A = R_1.A$ AND $R_3.B = R_4.B$ AND $R_2.B \neq R_3.B$ AND $R_1.A \neq R_4.A$
ORDER BY $R_1.A + R_4.A$ LIMIT k;
\end{lstlisting}

The query above seeks to find all author pairs who have appeared together in at least two different papers, ranked by the sum of their weights.~\autoref{enum:4cycle} shows the performance results for DBLP. Even to retrieve the top-$10$ results, all engines are slow and require expensive joins but \textsc{LinDelay} can find \emph{all} results within $2$ seconds.

==> introduction.tex <==
\section{Introduction} \label{intro}

Graph pattern extraction and analysis of the objects and their relationships in the underlying dataset provides insight and value in many application domains. Graph analysis tasks can perform anomaly and community detection in social media, fraud detection in finance, and data analysis for health monitoring, among many other applications. So far, the focus has been mostly on extracting full query results, i.e., queries that contain all join attributes in the selection clause of the query. Several key primitives, such as triangle and butterfly extraction~\cite{wang2020efficient}, wedge enumeration~\cite{santoso2020efficient}, and list intersections in web search engines~\cite{kim2018list} are examples of full patterns. In many cases, it is also required to rank the patterns in a specific order. This functionality is supported by the \sqlhighlight{ORDER BY} clause in \textsf{SQL} and \textsf{Cypher}. The following example demonstrates a practical use case.


\begin{example} \label{ex:1}
Consider the DBLP dataset as a single relation $R(A,B)$, indicating that $A$ is an author of paper $B$. Given an author $a$, function \textsf{h-index}$(a)$ returns the h-index of $a$. An analytical task involves accessing the relation through the following graph pattern: find all co-authors who authored at least one paper together. Additionally, the pairs of authors should be returned in decreasing order of the sum of their h-indexes, since users are only interested in the top-100 results. The following SQL query can capture this task.
	\lstset{upquote=true}
	
	\lstdefinestyle{mystyle}{
		commentstyle=\color{codegreen},
		keywordstyle=\color{codepurple},
		stringstyle=\color{codepurple},
		basicstyle=\small\ttfamily,
		breaklines=true,
		columns=fullflexible,
		frame=single,
	}
	\lstset{style=mystyle}
	
	\newcommand\numberstyle[1]{%
		
	}
	\begin{lstlisting}[ language=SQL,
	deletekeywords={IDENTITY},
	deletekeywords={[2]INT},
	morekeywords={clustered},
	mathescape=true,
	xleftmargin=0pt,
	framexleftmargin=0pt,
	frame=tb,
	framerule=0pt ]
	SELECT DISTINCT $R_1.A, R_2.A$ 
	FROM $R$ AS $R_1$, $R$ AS $R_2$
	WHERE $R_1.B = R_2.B$ 
	ORDER BY h_index($R_1.A$) + h_index($R_2.A$) 
	LIMIT 100;
	\end{lstlisting}
\end{example}

The above graph extraction task is an example of a non-full self-join pattern because the join attribute $B$ has been projected out. The \sqlhighlight{DISTINCT} clause ensures that there are no duplicate results. Such queries involving self-joins are prevalent in today's data analytical tasks~\cite{johnson2018towards} and have been extensively studied in the literature. 

\smallskip
\introparagraph{Previous Work} Efficient evaluation of graph queries (and more generally join queries) in the presence of ranking functions has been a subject of intense research in the database community (see~\autoref{sec:related} for a detailed overview). Recent work~\cite{tziavelis2020optimal, deep2019ranked} has made significant progress in identifying optimal algorithms for enumerating query results in ranked order. The performance metric for enumerating query results is the \emph{delay}~\cite{bagan2007acyclic}, defined as the time difference between any two consecutive answers. Prior work was able to obtain logarithmic delay guarantees, which were shown to be conditionally optimal. However, these results are only applicable to join queries \emph{without} projections. To apply existing algorithms to our setting, we need to convert the query with projections into a projection-free result. However, this conversion requires an expensive materialization step. For instance,~\autoref{ex:1} requires worst-case $\Omega(|D|^2)$ time and space (here $|D|$ is the size of the database) to materialize the join result of the query (without any ordering) before providing it as input for ranked enumeration. This motivates the development of new algorithms that avoid costly materialization and allow efficient enumeration.

On the practical side, all RDBMS and graph processing engines evaluate join queries with projections in the presence of ranking functions by performing three operations in serial order: $(i)$ materializing the result of the full join query, $(ii)$ de-duplicating the query result (since the query has \sqlhighlight{DISTINCT} clause), and $(iii)$ sorting the de-duplicated result according to the ranking function. The first step in this process is a show-stopper. Indeed, the size of the full join query result can be orders of magnitude larger than the size of the final output after applying projections and de-duplicating it. Thus, the materialization and the de-duplication step introduces significant overhead since they act as blocking operators. Further, if the user is interested in only a small fraction of the ordered output (top-$k$ with small $k$) -- expressed by the \sqlhighlight{LIMIT} clause -- the user still has to wait until the entire query completes even to see the top-ranked result. To make matters worse, the value of $k$ in the \sqlhighlight{LIMIT} clause is not even known until the user submits the query.

 \subsection{Our Contribution}   

In this paper, we initiate the study of ranked enumeration over join queries with projections (which we refer to as join-project queries below). We focus on two important ranking functions: \SUM\ ($f (x,z) = x+z$) and \lexi\ ($f (x,z) = x,z$) for two reasons. First, both of these functions are very useful in practice~\cite{ilyas2008survey}. Second, extending the algorithmic ideas to other functions, such as \sqlhighlight{MIN}, \sqlhighlight{MAX}, \sqlhighlight{AVG} and circuits that use sum and products, is quite straightforward. 
More specifically, we make three contributions. 

\smallskip
\introparagraph{1. Enumeration with Formal Delay Guarantees}
Our first main result shows that for any {\em acyclic} query (the most common fragment of queries in practice~\cite{bonifati2020analytical}) with arbitrary projection attributes, it is possible to develop efficient enumeration algorithms (\autoref{sec:acyclic}).

\begin{theorem} \label{thm:general}
	For an acyclic join-project query $Q$, an instance $D$ and a ranking function $\rank \in \{\text{\SUM}, \text{\lexi}\}$, the query result $Q(D)$ can be enumerated according to $\rank$ with worst-case delay $O(|D| \log |D|)$, after $O(|D|)$ preprocessing time.
\end{theorem} 

%Intuitively, relations in an acyclic query can be arranged in a tree-like fashion. 
This result implies that top-$k$ results in $Q(D)$ can be enumerated in $O(k |D| \log |D|)$ time.~\autoref{thm:general} is able to recover the prior results~\cite{deep2019ranked} for ranked enumeration of full queries as well. We are also able to generalize it to arbitrary join-project queries which may contain cycles using the idea of \emph{query decompositions}, as well as {\em union of queries},
%queries containing unions, 
which is a strictly more expressive class of queries.


\smallskip
\introparagraph{2. Faster Enumeration with More Preprocessing}
Our second contribution is an algorithm that allows for a smooth tradeoff between preprocessing time and delay guarantee for a subset of join-project queries known as {\em star} queries over binary relations of the form $R_i(A_i, B)$ (denoted as $Q^\star_m)$ (\autoref{sec:star}):

\lstset{upquote=true}

\lstdefinestyle{mystyle}{
	commentstyle=\color{codegreen},
	keywordstyle=\color{codepurple},
	stringstyle=\color{codepurple},
	basicstyle=\small\ttfamily,
	breaklines=true,
	columns=fullflexible,
	frame=single,
}
\lstset{style=mystyle}

\begin{lstlisting}[ language=SQL,
deletekeywords={IDENTITY},
deletekeywords={[2]INT},
morekeywords={clustered},
framesep=2pt,
mathescape=true,
xleftmargin=2pt,
framexleftmargin=1pt,
frame=tb,
framerule=0pt ]
SELECT DISTINCT $A_1, \dots, A_m$ FROM $R_1, \dots, R_m$
WHERE $R_1.B = \dots = R_m.B$ ORDER BY $A_1 + \dots + A_m$ LIMIT k;
\end{lstlisting}

Analysis of query logs has shown that star queries (both ranked and unranked) are the most important class of queries seen in practice that form over $90\%$ of all non-trivial queries in real world settings~\cite{bonifati2020analytical}. The main motivation of studying this setting as follows: for many data analysis pipelines, queries are asked repeatedly by users or accessed by some downstream tasks. In this case, it is desirable to spend some time {preprocessing} the input database in order to ensure that the repeated executions of the query are as fast as possible. The goal of the preprocessing phase is to compute a space-efficient intermediate data structure, which is used by the query answering algorithm to enumerate the query results according to an order given by a ranking function as fast as possible, and ideally, with delay guarantees.

\begin{theorem} \label{thm:ranked:star}
	For a star join-project query $Q^\star_m$, an  instance $D$, and a ranking function $\rank \in \{\text{\SUM}, \text{\lexi}\}$, the query result $Q(D)$ can be enumerated according to $\rank$ with worst-case delay $O\left(|D|^{1 - \epsilon} \log |D|\right)$, using $O\left(|D|^{1 + (m - 1) \epsilon}\right)$ preprocessing time and $O\left(|D|^{m(1 - \epsilon)}\right)$ space, for any $0 \leq \epsilon \leq 1$.
\end{theorem}

\autoref{thm:ranked:star} enables users to carefully control the space usage, preprocessing time and delay. For both~\autoref{thm:general} and~\autoref{thm:ranked:star}, we can show that the delay guarantee is optimal subject to a conjecture about the running time of star join-project queries in \autoref{sec:optimality}.

\smallskip
\introparagraph{3. Experimental Evaluation}
Our final contribution is an extensive experimental evaluation for practical join-project queries on real-world datasets (\autoref{sec:experiments}). To the best of our knowledge, this is the first comprehensive evaluation of how existing state-of-the-art relational and graph engines execute join-project queries in the presence of ranking. We choose MariaDB, PostgreSQL, two popular open-source RDBMS, and Neo4j, the most popular graph query engine, as our baselines. We highlight two key results. First, our experimental evaluation demonstrates the bottleneck of serially performing materialization, de-duplicating, and sorting. Even with \sqlhighlight{LIMIT 10} (i.e return the top-$10$ ranked results), the engines are orders of magnitude slower than our algorithm. For some queries, they cannot finish the execution in a reasonable time since they run out of main memory. On the other hand, our algorithm has orders of magnitude smaller memory footprint that allows for faster execution. Furthermore, the problem formulation in terms of delay guarantees allows our techniques to be limit-aware: for small values of $k$, the total answering time is also small. We empirically verify that as $k$ increases, the running time of the algorithm also increases proportionally. Although the theoretical delay of our algorithm is $O(|D| \log |D|)$, the empirical delay is smaller. The second key result is that all baseline engines are agnostic of the ranking function. The execution time of the queries is identical for both the sum and lexicographic ranking function. However, our algorithm uses the additional structure of lexicographical ordering and can execute queries $2-3\times$ faster than the sum function. For queries with unions and cycles, our algorithm maintains its performance improvement over the baselines. 
%
%\smallskip
%\introparagraph{Challenges of projections} We now discuss why evaluating queries with projections is challenging and how prior work is not. Consider the \emph{path query} with projections (a.k.a chain query in literature~\cite{bonifati2020analytical}): given $m$ binary relations of the form $R_i(x_i, x_{i+1})$, we define a path query  as follows:
%
%\lstset{upquote=true}
%
%\lstdefinestyle{mystyle}{
%	commentstyle=\color{codegreen},
%	keywordstyle=\color{codepurple},
%	stringstyle=\color{codepurple},
%	basicstyle=\small\ttfamily,
%	breaklines=true,
%	columns=fullflexible,
%	frame=single,
%}
%\lstset{style=mystyle}
%
%\newcommand\numberstyle[1]{%
%	
%}
%
%\begin{lstlisting}[language=SQL,
%	deletekeywords={IDENTITY},
%	deletekeywords={[2]INT},
%	morekeywords={clustered},
%	framesep=2pt,
%	mathescape=true,
%	xleftmargin=10pt,
%	framexleftmargin=40pt,
%	frame=tb,
%	framerule=0pt ]
%	SELECT DISTINCT $x_1,x_{m+1}$ FROM $R_1, \dots , R_m$
%	WHERE $R_1.x_2 = R_2.x_2$ AND $\dots$ AND $R_{m-1}.x_{m} = R_m.x_m$
%	ORDER BY $x_1+x_{m+1}$ LIMIT k;
%\end{lstlisting}
%
%
%The simplest path query for $m=2$, noted
%as $\twopath$, has a wide variety of applications (see~\cite{deep2020fast}). However, finding the optimal algorithm for evaluating $\twopath$ is already quite challenging, as $\twopath$ is equivalent to the boolean matrix multiplication (BMM) problem. Any improvement over the evaluation of $\twopath$ would imply the breakthrough on BMM problem, which is conjecture to be very difficult.  On the other hand, for arbitrary ranking functions,the trivial algorithm of materializing the full join results and then de-duplicating them by attributes $x_1,x_3$ is already optimal. 
%Moreover, de-duplicating query results (by the \sqlhighlight{DISTINCT} clause) introduces significant overhead, since state-of-the-art algorithms apply sorting or hashing on top of the full join results (with duplicates). As we will see later, our algorithm reduces this overhead significantly both in theory and practice,  by avoiding materializing full join results.  Finally, the  parameter $k$ could be part of the query, i.e., its value is not known in advance until the query has been issued by the user, so it will be harder for the query optimizer to find the best evaluation strategy without knowing $k$. In light of all these challenges above, it is no surprise that there is no efficient algorithm  known to enumerate query results in ranked order for join queries with projections. 
%
%Applying algorithms from prior work~\cite{tziavelis2020optimal, deep2019ranked} requires a full join query as input. However, converting a non-full join query requires polynomial time and space for materialization. For instance,~\autoref{ex:1} requires $\Omega(|D|^2)$ time and space in the worst-case to find the top ranked answer. This motivates the need to developing new algorithms that can avoid costly materialization and allow efficient enumeration.
%\xiao{How to apply previous work for ranked enumeration over full join queries to this settings? For free-connex query, there is a way to project non-output attributes out and obtain a weighted version of full join query.  But for non-free-connex query, there seems no way of avoiding materialization full join results. }
%
%
%\subsection{Our Results}   
%
%In this paper, we initiate the study of ranked enumeration over join queries with projections. We focus on two important ranking functions: \sum ($f (x,z) = x+z$) and \lexi ($f (x,z) = x,z$). for two reasons. First, both of these functions are very useful in practice~\cite{ilyas2008survey}. Second, extending the algorithmic ideas to other functions, such as \sqlhighlight{MIN}, \sqlhighlight{MAX}, \sqlhighlight{AVG} and circuits that use sum and products, is quite straightforward. The first main result of the paper shows that for any acyclic query (the most common fragment of join queries seen in practice~\cite{bonifati2020analytical}) with arbitrary projection variables, it is possible to achieve develop efficient enumeration algorithms. %Specifically, we show the following result (\autoref{sec:acyclic}).
%
%\begin{theorem} \label{thm:general}
%	For an acyclic join-project query $Q$, an instance $D$ and a ranking function $\rank \in \{\sum,$ $\lexi\}$,  there is an algorithm that can enumerate the query result $Q(D)$ according to $\rank$ with worst-case delay $O(|D| \log |D|)$, after $O(|D|)$ preprocessing time.
%\end{theorem}
%
%%Intuitively, relations in an acyclic query can be arranged in a tree-like fashion. 
%The result also implies that top-$k$ results in $Q(D)$ can be enumerated in $O(k \cdot |D| \cdot \log |D|)$ time. Our second result is to show a fine-grained algorithm that allows for a smooth tradeoff between preprocessing time and delay guarantee for a subset of acyclic queries known as {\em star} queries (denoted $Q^\star_m)$:
%
%\lstset{upquote=true}
%
%\lstdefinestyle{mystyle}{
%	commentstyle=\color{codegreen},
%	keywordstyle=\color{codepurple},
%	stringstyle=\color{codepurple},
%	basicstyle=\small\ttfamily,
%	breaklines=true,
%	columns=fullflexible,
%	frame=single,
%}
%\lstset{style=mystyle}
%
%\begin{lstlisting}[ language=SQL,
%	deletekeywords={IDENTITY},
%	deletekeywords={[2]INT},
%	morekeywords={clustered},
%	framesep=2pt,
%	mathescape=true,
%	xleftmargin=1pt,
%	framexleftmargin=1pt,
%	frame=tb,
%	framerule=0pt ]
%	SELECT DISTINCT $x_1, \dots, x_m$ FROM $R_1, \dots, R_m$
%	WHERE $R_1.y = \dots = R_m.y$ ORDER BY $x_1 + \dots + x_m$ LIMIT k;
%\end{lstlisting}
%%
%Analysis of query logs has shown that star and path queries (both ranked and unranked) are the most important class of queries seen in practice that form over $99\%$ of all non-trivial queries in real world settings~\cite{bonifati2020analytical}. For star queries, we show the following result:%(\autoref{sec:star}):
%
%\begin{theorem} \label{thm:ranked:star}
%	For a star join-project query $Q_m$, an  instance $D$, and a ranking function $\rank \in \{\sum,$ $\lexi\}$, there is an algorithm that can enumerate the query result $Q(D)$ according to $\rank$ with worst-case delay $O(|D|^q + \log |D|)$, using $O(|D|^p)$ preprocessing time and $O(|D|^{m \cdot (1-q)})$ space, where $p,q,m$ achieve the following tradeoff: %Let $O(|D|^p)$ denote the preprocessing time, $O(|D|^q + \log|D|)$ denote the delay guarantee for enumerating the query result according to the ranking function $rank$, and $O(|D|^s)$ denote the space requirement of the compressed data structure. Then, there exists a compressed data structure  and an algorithm with the following tradeoff:
%	{\small
%		\begin{align*}
%			p + (m-1) \cdot q &= m, \quad 0 \leq q \leq 1, p \ge 1% \\
%			%	s &= m \cdot (1-q)
%	\end{align*}}
%\end{theorem}
%
%The restriction on $p \ge 1$ is due to the fact that each input data must be read at least once.  Moreover, $p \le m$ since $O(|D|^{m})$ time is suffice to materialize the query results and sort them by $\rank$. %de-duplicate them by attributes $x_1, x_2, \cdots, x_m$ according to $\rank$. 
%%
%%Moreover, $p \leq m$ as we can always compute the full join and de-duplicate in time $O(|D|^k)$. 
%In addition, we also assume $0 \leq q \leq 1$ since linear delay can always be achieved for any acyclic query~\cite{bagan2007acyclic} (but only for unranked enumeration). For lexicographic ranking function, we can improve the result slightly by removing the log-factor from the delay. \autoref{thm:ranked:star} enables users to carefully control the space usage, preprocessing time and delay.  At last, this result also implies that the top-$k$ results of star query can be enumerated in 
%%of the data structure which in turn controls the delay guarantee. As before, the theorem implies that top-$k$ tuples in $Q^\star_m(D)$ can be enumerated in total time 
%$O(k \cdot |D|^q + k \cdot \log|D|)$ time.
%
%\smallskip \noindent
%%\introparagraph{A note on optimality} 
%{\bf Remark.} Building upon the conjecture on boolean matrix multiplication,  we can show that both~\autoref{thm:general} and~\autoref{thm:ranked:star} are optimal (\autoref{sec:optimality}) for a subset of CQs in \autoref{sec:optimality}.
%
%\smallskip
%
%At last, we implement our algorithm and compare it with state-of-the-art algorithms solutions in open-source (\textsf{MySQL} and \textsf{PostgreSQL}) and commercial databases (\textsf{Neo4J}) over real-world datasets. 
%All DBMS and graph engines used in the experimental evaluation deal with sum and lexicographic ordering in an extremely inefficient way; moreover their high cost of running time and space usage seem inherent even with \sqlhighlight{LIMIT 1}. Remarkably, our algorithm outperforms state-of-the-art solutions by $3 \times$ on average and up to three orders of magnitude in running time as well as space usage.


==> revision.tex <==
\onecolumn
\section*{Response Letter for Paper 227:  ``Ranked Enumeration of Join Queries with Projections''}
\label{sec:response}
We thank the reviewers for the revision opportunity and their clear, constructive reviews. To address the feedback, we have made major changes to the manuscript. Updates made in response to the comments are color-coded as follows. 


\begin{enumerate}
	\itemsep0em
	\item \ansm{Common changes for multiple reviewers and updates in the presentation of the paper are in RED.}
	\item \ansa{Reviewer 1 in PURPLE.}
	\item \ansb{Reviewer 2 in BROWN.}
	\item \ansc{Reviewer 3 in MAGENTA.}
\end{enumerate}


\subsection*{Meta-review}
	\ques{This paper studies ranked enumeration of join queries having projections. The authors mostly focus on acyclic queries, but extensions to cyclic queries can be also done. Although the paper is interesting, there are major concerns that are summarized as follows.} \\
	\ansm{We are thankful to all the reviewers and the meta-reviewer for the revision opportunity. We have significantly updated the paper to address all concerns raised by reviewers. To make room for the new material, we had to move some proofs and details to the Appendix.}\\

	\begin{enumerate}
		\item {\bf (Meta-review-1)} motivation is rather weak. Why do we care about join queries with projections in real scenarios? \\
		\ansm{We have updated the introduction and the related work to add motivation for why projection queries are important. Projection queries includes queries such as paths, reachability, matrix multiplication and play a critical role in problems such as set similarity and entity matching. Moreover, our results in this paper actually recover the algorithms from prior work as well which is a great benefit since a single unified algorithm is now able to capture full queries as well as non-full queries. }
		
		\item {\bf (Meta-review-2)} there are many presentation problems. \\
		\ansm{We have fixed all presentation issues. All typos, missing captions and orphans have been addressed. Some missing pieces and extra details have been added.} 
		
		\item {\bf (Meta-review-3)} empirical results should be strengthened. \\
		\ansm{We have added the following experiments to enhance our empirical studies:
		\begin{enumerate}
			\item Scalability experiments have been added.
			\item More datasets are added: we have clarified that the DBLP and IMDB datasets are actually multi-relational datasets and not graph datasets. Their schemas have also been added. Further, we have added 3 more large-scale datasets for experiments. Two of them are real-world and contain more than half a billion edges and we have also used LDBC social network benchmark.
			\item More practical queries are supported such as four cycle, six cycle etc. Motivation for all queries has also been added on why these are important.
			\item More choices of $k$ are tested.
	\end{enumerate}}
		
		\item {\bf (Meta-review-4)} many important technical issues are missing. \\
		\ansm{We have added many technical details in Section~\ref{sec:acyclic} and Section~\ref{sec:cyclic}. This includes all concerns raised by reviewer 1. We defer more detailed explanation to the section dedicated for each reviewer.
		}
\end{enumerate}
	

\subsection*{Reviewer 1}
\begin{enumerate}
	\item(R1-D1) \ques{In the introduction, it is not clarified why the related works on any-k queries [14, 18, 45, 47, 30, 12] are not suitable with projection. These works should be introduced with proper details, and the key challenges to answer any-k queries with projection should be discussed. Why prior works cannot be extended trivially to deal with projection?\\
	Then, some intuition must be given how the proposed method in this paper resolves this problem. The current introduction is not doing a good job in this regard.}\\
	\ansa{We have revamped the Introduction to address all of the concerns. We focus on the relational setting with graph only being an example use-case. We have now added a detailed discussion on why existing works are unable to handle the proposed problem and why trivial extensions are not enough to solve the problem.}
	
	\item(R1-D2) \ques{The introduction mainly talks about graph queries, however throughout the paper the data model used is relational, the query form and evaluation techniques are SQL-based. It is true that graph data can be represented in this form and graph queries could be answered via SQL, but that is not always natural. By graph queries, one may naturally think of pattern matching queries (e.g., pattern as a subgraph, triangle, path, clique, etc.) with labels on nodes and edges. Moreover, graph queries could be answered in a non-relational way, e.g., based on graph traversal and (exact or approximate) graph pattern matching, SPARQL queries, etc. Thus, the introduction must place the contribution of the paper in the right perspective. Graph queries could be shown as one interesting application/ case study, but probably not the key focus in this paper.} \\
	\ansa{We have changed the introduction to focus on the relation setting as suggested by the Reviewer.}
	
	\item(R1-D3) \ques{For cyclic queries, an exponential term is introduced, in the form $|D|^{\fhw}$, where "fhw" denotes fractional hypertree width. However, (a) "fhw" is not formally defined. (b) What are its values if a query pattern contains complex shapes and sizes, such as, triangles, cycles, cliques, bi-cliques, flowers, butterflies, etc.? (c) The exponential term also diminishes the technical contribution, unless it is shown that the complexities are tight. Formal proof on tightness must be provided.}\\
	\ansa{We have added the formal definition of $\fhw$ in \autoref{sec:framework} and several examples in Figure~\ref{fig:ghd}. The exponential term of \fhw\ (and \subw) is unavoidable in~\autoref{thm:cq} and~\autoref{thm:ucq} subject to popular conjectures (Combinatorial k-clique hypothesis proposed by~\cite{lincoln2018tight}). An unconditional lower bound is still out of reach and has been an open problem for at least $30$ years even for the simple triangle query. However, using the established conjectures, it can be shown that there exists queries for which the exponential term cannot be avoided. We have added a discussion in~\autoref{sec:cyclic}. The statement of the conjecture and the proof can be found in~\autoref{sec:finegrained}.}
	
	\item(R1-D4) \ques{In the general algorithm, how projection attributes are decided. Projection attributes should be query dependent. In Section-3.1, are they considering all possible sets of projection attributes? This could be huge space and time overhead.}\\
	\ansa{The reviewer is right that the projection attributes are query dependent. They are provided by the user (through the query). We believe the confusion was because of the sentence "all tuples over the subset of projection attributes that are present in the subtree rooted at node $i$." in the previous version that gives the impression that we are materializing tuples over all possible subset of projection attributes. \\
	
	This is not what the algorithm does. We have rephrased this sentence now. Once the join tree and its root is fixed, we are materializing tuples on *all* projection attributes in the subtree rooted at node $i$ and not all subsets of projection attributes. The set of projection attributes in the subtree at node $i$ (denoted using $A^\pi_i$) is a fixed set and we are not doing any operation over all possible subsets.
	}
	
	\item(R1-D5) \ques{How the root of the join tree is decided? Can any node be used as a root? Will the performance be impacted due to this choice?} \\
	\ansa{ We can use any node of the join tree as the root. All choices are valid and give the same worst-case time and space complexity. We empirically also tested the impact of this choice and found virtually no impact on the runtime performance (which is expected).
		
	The reviewer does bring up an interesting point on whether there is more performance to be extracted here. For more complex queries, one could envision taking both the query structure and data statistics into consideration. In this work, we focus on the worst-case complexity as the first step and we will go towards instance-optimal enumeration algorithm as our next step.
	}
	
	\item(R1-D6) \ques{"Note that the priority queue compares two cells based on their ranks on the
	output tuples formed and breaks ties according to the lexicographic ordering" --> why lexicographic ordering is used for tie breaking? Is this an arbitrary choice?}\\
	\ansa{Yes, using lexicographic ordering is an arbitrary choice. As long as the ties are broken consistently, other ranking functions can also be used.}
	
	\item(R1-D7) \ques{The data structures (e.g., cell, priority queue) used in the algorithms must be formally introduced (before discussing the algorithms). Their space complexities must be analyzed.}\\
	\ansa{We have now introduced the cell data structure and priority queue before the algorithms. Their space and time complexity is now explicitly mentioned.}
	
	\item(R1-D8) \ques{It must be formally proved that the proposed algorithms indeed return ranked results in correct order.}
	
	\ansa{We have added the formal proof in Lemma~\ref{lem:correctness} for the general algorithm,~\autoref{lem:lexi} for lexicographic algorithm and~\autoref{lem:star} for the star query. The full proofs are in the Appendix.}
	
	\item(R1-D9) \ques{It should be clarified that the "enumeration phase" is actually the online query phase.}
	
	\ansa{We have clarified this in Section~\ref{sec:problem-parameter} and in the abstract as well to highlight that the user queries are coming in an online fashion.}
	
	\item(R1-D10) \ques{What kind of ranking functions could not be handled (or, are difficult to deal with) for the proposed method, e.g., non-linear ranking functions?}
	
	\ansa{Ranking functions that do not have the "monotonicity" property are harder to handle in our framework. For example, $\rank(a,b) = |a - b|$ is a ranking function that is not monotone since it is decreasing and then increasing. We could handle this by breaking this function into multiple piecewise monotone function and then treat each piece separately. However, this requires some more bookkeeping and different techniques that are beyond the scope of the current work. This is an interesting extension that we plan to work on.}
	
	\item(R1-D11) \ques{In the experiments, only two small-scale graphs are used. Now-a-days, graph s with 100s of millions of nodes and billions of edges are publicly available. Moreover, in both datasets, only one binary relation exists, whereas throughout the paper, multiple relations are considered.}\\
	\ansa{We have clarified that the two small-scale datasets are actually multi-relational in nature. We have added their schema for clarity. Additionally, we have now also added 3 large scale datasets: two real-world datasets with more than $1B$ edges and the LDBC social network benchmark. We decided to keep the small-scale datasets for two reasons: first, none of the existing systems and DBMS engines are able to complete on the large- cale datasets. Therefore, in order to allow engines to finish execution we had to use a smaller dataset. Small datasets also allow for more fine-grained experimentation such as join ordering and experimenting with different weights (suggested by reviewer 2). Second, IMDB and DBLP are important datasets that have been used in prior work for analysis. 
		
	However, the reviewer is absolutely right that evaluation on large datasets is critical to strengthen the empirical results. We have added a section for experiments on large datasets.}
	
	\item(R1-D12) \ques{The queries are abstract and synthetic in nature. (a) They should be mapped properly to real-world query workloads/ benchmarks. (b) It is not clarified which attributes (e.g., A, B) are used in the context of real data, their selectivity, etc. and that impacts the query performance. (c) For cyclic queries, performance must be analyzed considering various sizes and shapes.}\\
	\ansa{We have now added the motivation for using the queries in the experiments and included the proper SQL statements as well. The queries are inspired by the multi-hop analysis frequently used in recommender systems and network analysis. For cyclic queries, we have chosen four important queries that have different shapes and used by prior work~\cite{tziavelis2020optimal}.
	}
	
	\item(R1-D13) \ques{The $k$ used is varied in the order of $10^6$ to $10^8$. However, in practice, the users may be interested only in top-10, or at most 100 answers in many real-world queries. So, the choice of $k$ should be properly justified and experiments must be conducted accordingly.}\\
	\ansa{ We have now added small $k$ to the experiments that show our performance is even better than for large $k$. The reviewer is right that users may be interested in small values of $k$. Our technique works well for both small and large $k$.}
	
	\item(R1-D14) \ques{Scalability experiments w.r.t. data size must be added.}\\
	\ansa{We have now added scalability experiments for the LDBC benchmark which is one of the large scale datasets. We run the experiments for multiple scale factors and show that our technique is scalable.}
	
	\item(R1-D15). \ques{Many presentation issues:
	(a) the paper exceeds the page limit (12 pages without references). This could even be a reason for desk-reject.
	(b) many orphan words.
	(c) "our work paves the way forward for building truly nonblocking operators for graph query processing, allowing for better pipelining when the output can stream through multiple tasks." --> It is not clear how such generalization is made at the end of introduction.
	(d) "query results results" --> query results} \\
	\ansa{All the presentation issues are now addressed. We sincerely apologize for these errors and thank the reviewer for their careful reading of the manuscript.}

\end{enumerate}

\subsection*{Review 2}
\begin{enumerate}
	\item(R2-D1) \ques{Why we need consider join queries with projections? Will it bring some benefits? The motivation of using projections for join queries should be strengthened in the introduction.
	In addition, in database sql, we can used some techniques, such join orders, to accelerate the processing, instead of do the natural join first and then do the other operations. Especially for the ranking problem, it will greatly reduce the candidate space. Authors should be provide more discussion about this part and it would be better to provide some experimental evaluation regrading this issue.}\\
	\ansb{We have revamped the introduction to add motivation for projections for join queries and why it is important.
	The reviewer brings up an excellent point about exploring join ordering for faster query execution. We have added a subsection in the experiments to explore the impact of different join orderings. The idea is that there may be a join order that leads to improved query execution time and the DBMS engine could applying the ordering function more effectively. Unfortunately, we observed that the best join order still leads to less than $2\%$ reduction in query execution time. The problem with join ordering is that while the query execution may become faster, the bottleneck of materialization still remains which is the dominant cost. Therefore, the benefit of join ordering is not visible. Further, when we have self-joins, all join orderings are identical since all relations are the same.

	But since our algorithm is a type of multi-way join where ranking is fused into the join operator itself, we do not need any join ordering exploitation. We believe that the idea exploiting join orderings may actually be very useful in the case of approximate ordering instead of exact ordering but that problem requires a much deeper investigation and beyond the scope of the current paper.}
	
	\item(R2-D2) \ques{In the experiments, only binary relations are considered. It would be better to provide the experiments with more complex relations to verify the performance of developed techniques.For the weight of the datasets, it would be better to consider different weight distribution, and more datasets should be used to verify the performance.}\\
	\ansb{We clarify that the IMDB and DBLP datasets are actually multi-relational in nature. We have added their schemas as well. We have also added 3 large scale datasets and verify that our techniques work very well on larger sized datasets too. For the weights, we have now used two types of weights: first is random weights and the second is weights in proportion to the degree of the tuples. This function has been proposed in existing literature. We have added a paragraph in the experimental section to present our findings.}
	
	\item(R2-D3) Proofreading is required. In Example 2, it should be R4 (a leaf node) instead of R3.The Figure 2 has only the figure but lacks the corresponding caption. There are some typos, such as the query results results and to the the first extensive. 
	
	\ansb{All presentation issues have been fixed. We thank the reviewer for a detailed reading and pointing these out.}
	
\end{enumerate}

\subsection*{Review 3}

\begin{enumerate}
	
	\item (R3-W1) In the related work, the differences between the proposed problem and existing queries are not clarified well enough.
		
	\ansc{We have now highlighted the differences between our work and prior work in the related work section. In each subsection, we explicitly state the weakness of prior work and how this paper solves those issues.}
	
	\item (R3-W2) The algorithms developed in this paper are in memory oriented. However, in this big data era, external memory or distributed database systems are more common and practical. Thus, can the proposed algorithms be extended to these settings. If not, what are the major obstacles.
	
	\ansc{This is an interesting research topic. In order to extend our results, we need to investigate how to partition the data optimally so that each distributed node can perform execution and then be efficiently combined. A key challenge in that space is to analyze how we can balance the load so that no node is overwhelmed and each distributed node actually generates the output efficiently. We have added a discussion on this in the conclusion on this and stated it as an open problem.}
	
\end{enumerate}


